Parameterization of Electron Attachment Rate Constants for Common Impurities in LArTPC Detectors

The ability of free electrons to drift long distances at high velocities in pure liquid argon under an applied electric field has been exploited for the past forty years to implement detectors with increasingly large volumes for high energy physics research. In this paper, we summarize the electron attachment rate constants as a function of the external electric field for common impurities in LArTPC with data from the literature. We further provide analytical functions to parameterize the data, which are useful to compare with new measurements as well as to make extrapolations.

==> Makefile <==
########################################################################
#
# $Id: Makefile,v 1.2 2010/10/29 15:06:33 slavic Exp $
#
##########################################################################
TEX = pdflatex
BIB = bibtex
#main file
texfile = TS_JINST
#all figures
FIGS=$(wildcard figures/*.*)
#all texfiles
SECS=$(wildcard ./*.tex)
#SECS=$(wildcard sections/*.tex)

export TEXINPUTS:=$(CURDIR):$(CURDIR)/ar2estyle:$(TEXINPUTS)
export BSTINPUTS:=$(CURDIR):$(CURDIR)/ar2estyle:$(BSTINPUTS)
export BIBINPUTS:=$(CURDIR):$(CURDIR)/ar2estyle:$(BIBINPUTS)

.PHONY: pdf
.PHONY: clean

all: pdf

pdf: $(texfile).pdf

$(texfile).pdf : $(SECS) $(texfile).tex $(texfile).bib #$(FIGS) 
	$(TEX) $(texfile)
	$(BIB) $(texfile) # compile bibliography
	$(TEX) $(texfile)
	$(TEX) $(texfile)

clean:
	@ls $(texfile).* | grep -v '.tex\|.bib' | xargs -I {} rm {}

